2nd Place Solution for MOSE Track in CVPR 2024 PVUW workshop: Complex Video Object Segmentation

Complex video object segmentation serves as a fundamental task for a wide range of downstream applications such as video editing and automatic data annotation. Here we present the 2nd place solution in the MOSE track of PVUW 2024. To mitigate problems caused by tiny objects, similar objects and fast movements in MOSE. We use instance segmentation to generate extra pretraining data from the valid and test set of MOSE. The segmented instances are combined with objects extracted from COCO to augment the training data and enhance semantic representation of the baseline model. Besides, motion blur is added during training to increase robustness against image blur induced by motion. Finally, we apply test time augmentation (TTA) and memory strategy to the inference stage. Our method ranked 2nd in the MOSE track of PVUW 2024, with a $\mathcal{J}$ of 0.8007, a $\mathcal{F}$ of 0.8683 and a $\mathcal{J}$\&$\mathcal{F}$ of 0.8345.

==> sec/2_method.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=0.95\linewidth]{fig/Fig 2.pdf}
   \caption{Architecture of Cutie.}
   \label{fig:2}
\end{figure*}
\FloatBarrier

\section{Method}
\label{sec:method}

As illustrated in \cref{fig:1}, our solution takes Cutie as the baseline model. Then, we use instance segmentation and motion blur to augment the training data. Finally, during the inference stage, we employ TTA and memory strategies to improve the results. Details of the solution are described as follows. 

%-------------------------------------------------------------------------
\subsection{Baseline model}
To ensure good performance under challenges such as frequent disappearance-reappearance, heavy occlusions, small and similar objects, we introduces Cutie as the strong baseline model, as shown in \cref{fig:2}. Cutie stores a high-resolution pixel memory $F$ and a high-level object memory $S$. The pixel memory is encoded from the memory frames and corresponding segmented masks. The object memory compresses object-level features from the memory frames. When a new query frame comes, it bidirectionally interacts with the object memory in a couple of object transformer blocks. Specifically, given the feature map of the query frame, the pixel readout $R_0$ is extracted by reading from the pixel memory with a sensory memory[XMem], then the pixel readout interacts with the object memory and a set of learnable object queries through bottom-up foreground-background masked cross attention. Next, the obtained high-level object query representation communicates back with the pixel readout through top-down cross attention. The output pixel readout $R_l$ and object queries $X_l$ are sent to the next object transformer block. The final pixel readout will be combined with multi-scale features passed from skip connections for computing the output mask in the decoder. Cutie enriches pixel features with object-level semantics in a bidirectional fashion, hence is more robust to distractions such as occlusion and disappearance. 

\subsection{Data augmentation}
Like most state-of-the-art VOS methods, Cutie also adopts a two-stage training paradigm. The first stage pretraining uses short video sequences generated from static images. Then main training is performed using VOS datasets in the second stage. However, the original Cutie fails to perform well when similar objects move in close proximity or suffers from serious motion blur. 

To solve the above problems, we conduct data augmentation to enhance the training of Cutie. First, we employ the universal image segmentation model Mask2Former to segment instance targets from the valid set and test set of MOSE. As shown in the left column of \cref{fig:3}, the segmented small objects represent typical object appearances in MOSE, which is helpful for learning the semantics of diverse objects in advance. Meanwhile, as shown in the middle column of \cref{fig:3}, we convert the instance annotations of COCO[] into independent binary masks. Here we select object classes such as human, animal and vehicle that frequently occur in MOSE to reduce  discrepancy between \begin{figure*}
    \centering
    \begin{tabular}{c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c}
    \includegraphics[width=0.32\linewidth, height=0.20\linewidth]{fig/Fig 3/mose-test.jpg} & 
        \includegraphics[width=0.32\linewidth, height=0.20\linewidth]{fig/Fig 3/coco.jpg} & 
        \includegraphics[width=0.32\linewidth, height=0.20\linewidth]{fig/Fig 3/bike.jpg} \\
        \includegraphics[width=0.32\linewidth, height=0.20\linewidth]{fig/Fig 3/mose-test.png} & 
        \includegraphics[width=0.32\linewidth, height=0.20\linewidth]{fig/Fig 3/coco.png} & 
        \includegraphics[width=0.32\linewidth, height=0.20\linewidth]{fig/Fig 3/bike_blur.jpg} \\
     \end{tabular}
    \caption{Examples of generated pretraining data and motion blur. Left: binary mask generated from the valid set and test set of MOSE. Middle: binary mask generated from COCO, the masks of different classes are merged into one mask. Right: example of motion blur in the horizontal direction.}
    \label{fig:3}
\end{figure*}
\FloatBarrier 
\noindent two data distributions. The acquired data is used as extra pretraining data to enable more robust semantics and improve discrimination ability against diverse objects of MOSE. Second, with the observation that motion blur is a significant challenge, we add motion blur with random kernel sizes and angles to both the pretraining and main training stages. An example of motion blur is shown in the right column of \cref{fig:3}. The proposed data augmentation aims at training towards better robustness and generalization. 

\subsection{Inference time operations}
During inference, we introduces TTA and memory strategies to further increase the performance.
\textbf{TTA.} We use two kinds of TTA: flipping and multi-scale data enhancement. We only conduct horizontal flipping since experiments show flipping in other directions is detrimental to performance. In addition, we inference results on the test set under three maximum shorter side resolutions: 600p, 720p and 800p. The multi-scale results are then averaged to get the final result.\\
\textbf{Memory strategies.} We find in experiments that larger memory banks and shorter memory intervals lead to better performance. Therefore, we adjust the maximum memory frames $T_{\max}$ to 18 and the memory interval to 1. 

